How to Count Triangles, without Seeing the Whole Graph

Triangle counting is a fundamental problem in the analysis of large graphs. There is a rich body of work on this problem, in varying streaming and distributed models, yet all these algorithms require reading the whole input graph. In many scenarios, we do not have access to the whole graph, and can only sample a small portion of the graph (typically through crawling). In such a setting, how can we accurately estimate the triangle count of the graph? We formally study triangle counting in the {\em random walk} access model introduced by Dasgupta et al (WWW '14) and Chierichetti et al (WWW '16). We have access to an arbitrary seed vertex of the graph, and can only perform random walks. This model is restrictive in access and captures the challenges of collecting real-world graphs. Even sampling a uniform random vertex is a hard task in this model. Despite these challenges, we design a provable and practical algorithm, TETRIS, for triangle counting in this model. TETRIS is the first provably sublinear algorithm (for most natural parameter settings) that approximates the triangle count in the random walk model, for graphs with low mixing time. Our result builds on recent advances in the theory of sublinear algorithms. The final sample built by TETRIS is a careful mix of random walks and degree-biased sampling of neighborhoods. Empirically, TETRIS accurately counts triangles on a variety of large graphs, getting estimates within 5\% relative error by looking at 3\% of the number of edges.

==> source/old-algo.tex <==
\section{The Main Result and \ALG}
In this section, we present and analyze our triangle counting algorithm
\ALG~\cref{alg:triangle_estimate}. 
% We first state a
% more detailed version of our main theorem.
% \begin{theorem}
% \label{thm:main}
% Let $\eps,\delta \in[0,1]$ be some constants and $\overline{m}$ be an
% estimate for $m$ such that $(1-\eps)m \leq \overline{m} \leq (1+\eps)m$.
% Then \ALG is an $(\eps,\delta)$-estimator
% to the triangle count while making
% \begin{align*}
% O\left(\log \left(\frac{1}{\delta}\right) \frac{\log n}{\eps^2}
% \left( \frac{m \mix \nt_{\emax}}{\NT} + \frac{m \alpha} {\NT} \right) \right)
% \end{align*}
%  many queries.
% \end{theorem}
% We first describe our algorithm \ALG. The pseudo code for 
% \ALG is given in~\cref{alg:triangle_estimate}. 
It takes
two input parameters: the length of the random walk $\wL$,
and the number of subsamples (explained below) $\sL$.
\ALG starts with a arbitrary vertex of the graph provided by the model.
Then it performs a random walk of length $\wL$ and collect the
edges in a ordered multi-set $R$. For each edge $e =\{u,v\}\in R$,
it computes the degree $d_e$. Recall the definition
of degree of an edge: $d_e= \min \{d_u,d_v\}$. 
In the next step, \ALG sample an edge from $R$ proportional to its
degree. The parameter $\sL$ dictates the number of independent samples
to be drawn from $R$ according to the edge degree distribution.

For an edge  $e$ sampled in the above step, \ALG
samples a neighbor $w$ from $N(e)$, u.a.r.; recall $N(e)$ denote the neighbors of the lower degree end point. Such an sample is acquired by making a random neighbor query from the lower degree end point of $e$. Finally, using edge queries, \ALG checks whether a
triangle is formed by $\{e,w\}$. If it forms a triangle, 
\ALG check
if the triangle in uniquely assigned to the edge $e$ (see~\Cref{sec:prelim} for the assignment rule).

To compute the final estimate for triangles, \ALG requires 
a good estimate for the number of edges. Recall that
the total number of edges is not readily available in our model.
To accomplish this task, we design a collision based edge estimator
in~\Cref{alg:edge_estimate}, based on a result of Ron and Tsur~\cite{RT16}.


\begin{algorithm}[!ht]
\caption{\ALG --- Triangle Counting Estimator}
\label{alg:triangle_estimate}
    \begin{algorithmic}[1]
    \Procedure{\ALG}{$\wL$, $\sL$}
    \label{proc:EstTri}
    \State Let $\seed$ be some arbitrary vertex provided by the model.
    \State Let $R$ be the multiset of edges on an $\sL$-length random walk from $\wL$.
    \For {$i=1$ to $\sL$} \label{line:loop}
    \State Sample an edge $e\in R$ independently with prob. $d_e/d_R$.
    \State Query a uniform random neighbor $w$ from $N(e)$.
    \State Using edge query, check if $\{e,w\}$ forms a triangle.
    \State If $\{e,w\}$ forms a triangle $\tau$: query for degrees of all vertices
    in $\tau$ and determine if $\tau$ is associated to $\{e,w\}$.
    \State If $\tau$ was associated to $\{e,w\}$, set $Y_i=1$; else set $Y_i=0$.
    \EndFor
    \State Set $Y = \frac{1}{\sL} \sum_{i=1}^{\ell} Y_i$. \label{line:Y}
    \State Let $\overline{m}$ = \textsc{EdgeCountEstimator}$~(R,\mix)$
    \State Set $X = \frac{\overline{m}}{\wL} \cdot d_R \cdot Y$.
    \State return $X$.
    \EndProcedure
%     \Procedure{RandomWalk}{vertex $\seed$, integer $\wL$} \label{proc:rand_walk}
%     \State $u \gets \seed$
%     \For {$i=1$ to $\wL$}
%     \State Query for a uniform random neighbor of $v\in N(u)$.
%     \State $e_i \gets \{u,v\}$.
%     \State $u \gets v$.
%     \EndFor
%     \State Let $R=(e_i)_{i=1}^{r}$ be the ordered (multi)-set edges.
%     \State return $R$.
%     \EndProcedure
%     \Procedure{IsAssociated}{$\tau=\{e=\{u,v\},w\}$}
%     \label{proc:isAsso}
%     \If {$u \prec_{\deg} w$ and $v \prec_{\deg} w$}
%     \State return YES.
%     \Else 
%     \State return NO.
%     \EndIf
%     \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{Edge Count Estimator}
\label{alg:edge_estimate}
    \begin{algorithmic}[1]
    \Procedure{\textsc{EdgeCountEstimator}}{edge set $R$, integer $\mix$}
        \label{proc:EstEdge}
        \For {$i=1$ to $\mix$}
        \State Let $R_i = (e_i,e_{i+\mix},e_{i+2\mix},\ldots)$. \label{line:R_i)}
        \State Set $c_i=$number of pairwise collision in $R_i$.
        \State Set $Y_i= \binom{|R_i|}{2} / c_i$.
        \EndFor
        \State Set $Y=\frac{1}{\mix} Y_i$.
        \State return $Y$.
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\subsection{Theoretical Analysis of \ALG}
We provide a theoretical analysis of \ALG and prove ~\cref{thm:tri_count}. 
We first show that if the collection of edges $R$ exhibits some ``nice" properties, then
we have an accurate estimator. Then we prove that the collection of edges 
$R$ produced by random walk has these desired properties.
Our goal is to prove that the output of
\ALG, $X$, is an $(\eps,\delta)$-estimator for the triangle counts.
For ease of exposition, in setting parameter values of 
$\wL$  and $\sL$, we hide the dependency
on the error probability $\delta$. A precise calculation
would set the dependency to be $\log (1/\delta)$, as standard
in the literature.

We first show that the random variable $Y$ (~\cref{line:Y})
roughly captures the ratio $\NT/d_E$. To show this,
we first fix an arbitrary collection of edges $R$,
and simulate \ALG on it. We show that, in expectation,
$Y$ is going to $t_R/d_R$. For the sake of clear presentation,
we denote the value of the random variable $Y$, when run
with the edge collection $R$, to be $Y_R$. Note that, $Y_R$
is a random variable nevertheless; the source of the
randomness lies in the $\sL$ many random experiments that
\ALG does in each iteration of the for loop at ~\cref{line:Y} of ~\Cref{alg:triangle_estimate}
\begin{lemma}
\label{lem:triangle_est}
Let $R$ be a fixed collection of edges, and $Y_R$ denote the value of the random variable $Y$ on the fixed set $R$ (~\cref{line:Y} of ~\Cref{alg:triangle_estimate}).  Then,
\begin{enumerate}
    \item $\EX [Y_R] = \frac{\nt_R}{d_R}$,
    \item $\Pr \left[~|Y_R - \EX[Y_R]| \geq \eps \EX [Y_R]~ \right] 
    \leq \exp \left( - \sL \cdot \frac{\eps^2}{3} \cdot \frac{\nt_R}{d_R}  \right)$.
\end{enumerate}
\end{lemma}
\begin{proof}
We first prove the expectation statement. 
Let $e_i$ be the random variable that denotes the edge sampled
in the $i$-th iteration of the for loop (~\cref{line:loop}).
Consider the random variable $Y_i$.
We have
\begin{align*}
    \Pr[Y_i=1] &= \sum_{e\in R} \Pr[e_i = e]\Pr [Y_i =1 | e_i = e] \,,  \\
    &= \sum_{e\in R} \frac{d_e}{d_R} \Pr [Y_i =1 | e_i = e] = \sum_{e \in R} \frac{\nt_e}{d_R} = \frac{\nt_R}{d_R} \,.
\end{align*}
Where the second last equality follows as for a fixed edge $e$, the probability that $Y_i=1$ is exactly $t_e/d_e$.
Since $Y= (1/\sL) \sum_{i=1}^{\sL} Y_i $,
by linearity of expectation, we have the item (1) of the lemma.

For the second item, we apply Chernoff bound(~\cref{thm:chernoff}).
\end{proof}

Clearly, for any arbitrary set $R$, we may not have the desired
behavior of $Y$ that it concentrates around $\NT/d_E$. 
To this end, we first define the desired properties of $R$ and
then show \ALG produces such a edge collection $R$ with high 
probability.
\begin{definition}[A {\em good} collection of edges]
We call a edge collection $R$ {\em good}, if it satisfies the 
following two properties:
\begin{align}
    &\frac{\nt_{R}}{d_R} \ge (1-\eps) \cdot \frac{\eps}{\log n} \cdot \frac{\NT}{d_E} \label{eqn:prop_1} \\
    & \nt_R \in \left[ (1-\eps) |R| \cdot \frac{\NT}{m} ~~,~~  (1+\eps) |R| \cdot \frac{\NT}{m} \right] \label{eqn:prop_2}
\end{align}
\end{definition}
For now we assume the edge collection $R$
produced by \ALG is {\em good}. Observe that,
under this assumption, the expected value of 
$Y_R$ is  $\nt_R/d_R \geq \tO(\NT/d_E)$. In the next lemma, we 
show that for the setting of $\sL= \tO(d_E/\NT)$, $Y_R$
concentrates tightly around its mean.

\begin{lemma}%[Concentration of {\em good} $R$]
\label{lem:goodY}
Let $0 < \eps < 1/2$ and $c>6$ be some constants, and $\sL = \frac{c \log^2 n}{\eps^3}\cdot \frac{d_E}{\NT}$. 
Conditioned on $R$ being {\em good}, 
with probability at least $1- o(1/n)$, 
$|Y_R - \EX[Y_R]| \leq \eps \EX[Y_R] $.
\end{lemma}
\begin{proof}
Since $R$ is {\em good}, by the first property (~\cref{eqn:prop_1}),
we have 
$\frac{t_R}{d_R} \geq (1-\eps) \cdot \frac{\eps}{\log n} \cdot \frac{\NT}{d_E} $. 
Then, by item (2) in~\Cref{lem:triangle_est}, we have
\begin{align*}
    &\Pr \left[~|Y_R - \EX[Y_R]| \geq \eps \EX [Y_R]~ \right] \\
    & \leq \exp \left( - \frac{c \log^2 n}{\eps^3}\cdot \frac{d_E}{t} 
    \cdot\frac{\eps^2}{3} \cdot (1-\eps) \cdot \frac{\eps}{\log n} \cdot \frac{t}{d_E}  \right) \,,\\
    &= \frac{1}{n^ {\frac{c(1-\eps)}{3}}}\,,
\end{align*}
where the second inequality follows by plugging in the values of $\sL$.
The lemma follows by the constraints on the values of $c$ and $\eps$.
\end{proof}

We now show that, conditioned on $R$ being {\em good},
the final estimate $X$ is lies between
$(1-4\eps)\NT$ and $(1+4\eps)\NT$ with high probability. We later
remove the conditioning on $R$ by showing that with high probability,
\ALG produces a {\em good} $R$.
\begin{lemma}
\label{lem:tri}
Condition on the event that $R$ is good. Then,
with probability at least $1-o(n)$, 
$X_R \in [(1-4\eps t), (1+4\eps t)]$.
\end{lemma}
\begin{proof}
Recall that $\EE[Y_R] = \nt_R /d_R$.
Conditioned on the  event of $R$ being good,
with probability at least $1-o(n)$, $Y_R$ is closely
concentrated around its expected value (~\Cref{lem:goodY}).
Hence, we have
\begin{align*}
    Y_R \in \left[(1-\eps) \frac{\nt_R}{d_R}~~,~~ (1+\eps) \frac{\nt_R}{d_R} \right] \,.
\end{align*}
Now consider the final estimate $X$. For a fixed set $R$, denote
the value of the random variable $X$ to be $X_R$. Note that,
$X_R$ itself is a random variable where the source of the
randomness is same as that of $Y_R$. More importantly,
$X_R$ is a just a scaling of the random variable $Y_R$:
$X_R = (\overline{m}/\wL)\cdot d_R \cdot Y_R$.
Then, with high probability
\begin{align*}
    X_R \in \left[\frac{\overline{m}}{\wL} \cdot d_R \cdot (1-\eps)\cdot  \frac{\nt_R}{d_R} ~~,~~ \frac{\overline{m}}{\wL} \cdot d_R \cdot (1+\eps) \cdot  \frac{\nt_R}{d_R} \right] \,.
\end{align*}
Simplifying we get, with high probability,
\begin{align*}
    X_R \in \left[(1-\eps) \cdot \frac{\overline{m}}{\wL} \cdot  {\nt_R}~~,~~ (1+\eps) \cdot  \frac{\overline{m}}{\wL} \cdot {\nt_R} \right] \,.
\end{align*}
Since $R$ is good, by using the second property (~\cref{eqn:prop_2}), 
and putting $|R|=r$
\begin{align*}
    X_R \in \left[(1-2\eps) \cdot \frac{\overline{m}}{m} \cdot  {\NT}
    ~~,~~ (1+2\eps) \cdot  \frac{\overline{m}}{m} \cdot {\NT} \right] \,.
\end{align*}
By assumption, $\overline{m} \in [(1-\eps)m~~,~~(1+\eps)m]$. Hence,
with probability at least $1-o(n)$,
$X_R \in \left[ (1-4\eps) \NT, (1+4\eps)\NT  \right]$.
This completes the proof of the lemma.
\end{proof}

In the remaining part of this section, we focus on
removing the condition on $R$ from the~\Cref{lem:tri}. 
In this regards, we show that with probability at least $1-1/4\log n$,
the edge collection produced by \ALG is {\em good}.
This would completes the proof of our main result.

We now analyze the properties of the edge (multi)set 
$R$ collected by a random walk. 
For our theoretical analysis,
we first ignore the first $\mix$ many steps in $R$.
Abusing notation, we reuse $R$ to denote the remaining edges.
We denote sum of degrees of the edges in $R$ by $d_R=\sum_{e\in R} d_e$.
In a similar vain, we denote by $\nt_R$ the sum of the triangle count
of the edges in $R$: $\nt_R = \sum_{e \in R} \nt_{e}$.
In the next lemma, we prove that the random variables $d_R$
and $\nt_R$ are tightly concentrated around their mean.

\begin{lemma}[Analysis of \textsc{RandomWalk}]
\label{lem:good_set}
Let $\eps>0$ and $c>6$ be some constants, and $\wL = \frac{\log n }{\eps^2}\cdot \frac{m \mix  \nt_{\emax}}{\NT}$. Let $R$, $d_R$, and $\nt_{R}$ be as defined above. Then,
\begin{enumerate}
    \item $\EX[d_R] = |R| \cdot \frac{d_{E}}{m} $ and $\EX [{\NT}_R] = |R|\cdot  \frac{\NT}{m} $.
    \item With probability at least $1-\frac{\eps}{\log n}$, $d_R \leq \EX \left[ d_R \right] \cdot \frac{\log n}{\eps}$.
    \item With probability at least $1-\frac{1}{c\log n}$, 
    $|\nt_R -\EX[\nt_R]| \leq \eps \EX[\nt_R] $.
\end{enumerate}
\end{lemma}
We defer the proof of ~\Cref{lem:good_set} and first 
show how does this lemma, combined with~\Cref{lem:tri},
prove our main theorem.
\begin{proof}[Proof of~\Cref{thm:main}]
\Cref{lem:good_set} implies, with probability at least 
$1-1/4\log n$, we have $\nt_R \geq (1-\eps) \cdot |R| \cdot \frac{\NT}{m}$
and $d_R \leq \frac{\log n}{\eps }\cdot |R| \cdot \frac{d_E}{m}$.
Hence,
\begin{align*}
\frac{\nt_R}{d_R} \geq (1-\eps) \cdot \frac{\eps}{\log n} \cdot \frac{\NT}{d_E} 
\end{align*}
This is the first property (~\cref{eqn:prop_1}) for $R$ to 
to be {\em good}. The second property (~\cref{eqn:prop_2}) is true by the item (3) of ~\Cref{lem:good_set}. Hence, $R$ is {\em good} with
probability at least $1-1/4\log n$. Hence, we remove the
condition on~\Cref{lem:tri}, and derive that with probability at least
$1-1/3\log n$,
$    X \in \left[ (1-4\eps) \NT, (1+4\eps)\NT  \right]$.
Re-scaling the parameter $\eps$ appropriately, the accuracy of 
\ALG follows. The number of queries is bounded by $O(\wL+\sL)$.
The query bound of the theorem follows by applying~\Cref{lem:chiba}, .
\end{proof}
We now prove the last piece --- ~\Cref{lem:good_set}.
\begin{proof}[Proof of ~\Cref{lem:good_set}.]
We first compute the expected value of $d_R$ and $\nt_R$. 
For each index $i\in [|R|]$ in the set $R$, we define two random variables $Y_{i}^{d}$ and $Y_{i}^{\NT}$:
$Y_{i}^{d} = d_{e_i}$, and $Y_{i}^{\NT} = \nt_{e_i}$, where 
$e_i$ is the $i$-th edge in $R$. 
Then, $d_R = \sum_{i=1}^{\wL'} Y_{i}^{d}$ and $t_R = \sum_{i=1}^{\wL'} Y_{i}^{\NT}$. We have
\begin{align*}
    \EX \left[Y_{i}^{d} \right] &= \sum_{e \in E} \Pr[e_i=e] \cdot \EX 
    \left[ Y_{i}^{d} | e_i = e\right] = \frac{1}{m} \sum_{e \in E} d_e = \frac{d_{E}}{m} \,.
\end{align*}
Then, by linearity of expectation, we get $\EX [d_R] = |R| \cdot {d_{E}}/{m} $.
Analogously, using the fact that $\sum_{e\in E}\nt_e = \NT$, we get $\EX [\nt_R] = |R|\cdot  \NT /m $. 

We now turn our focus on the concentration of $d_R$. This is achieved by a simple application of Markov inequality.
\begin{align*}
    \Pr \left[ d_R \geq \EX \left[ d_R \right] \cdot \frac{\log n}{\eps} \right] \leq \frac{\eps}{\log n} \,.
\end{align*}
Hence, the second item in the lemma statement follows.

We now prove the third item. To prove a concentration bound on $\nt_R$, 
we fist bound the variance of $\nt_R$ and then apply Chebyshev
inequality~\cite{Alsmeyer2011}. Note that not all the edges in $R$
are independent --- however, the edges that
are at least $\mix$ many steps apart in the set $R$ are
independent. So we break the variance computation into two parts
as follows:
\begin{align*}
    &\Var[\nt_R] = \EE[\nt_R^2] - \left(\EE[\nt_R]\right)^2 \\
    &= \sum_{|i-j|> \mix} \EE[Y_{e_i}]\cdot \EE[Y_{e_j}] + \sum_{|i-j|\leq  \mix} \EE[Y_{e_i}\cdot Y_{e_j}] - \left(\EE[\nt_R]\right)^2  \\
    &\leq  \left(\EE[\nt_R]\right)^2 + \sum_{i\in [|R|]} \mix \cdot \nt_{\emax} \cdot \EE[Y_{e_i}]
    -\left(\EE[\nt_R]\right)^2  \\
    & \leq \mix \cdot \nt_{\emax} \cdot |R| \cdot \frac{\NT}{m}\,.
\end{align*}
Then, by an application of Chebyshev inequality (~\cite{Alsmeyer2011}), we get
\begin{align*}
    \Pr [ |\nt_R -\EX[\nt_R]| &\geq \eps \EX[\nt_R] ]  \,, \\
    & \leq \frac{\Var[t_R]}{\eps^2 \EX[\nt_R]^2} \,, \\
    &= \frac{1}{\eps^2}\cdot \frac{ \mix \cdot \nt_{\emax} \cdot |R| \cdot \NT }{m}
        \cdot \frac{m^2}{|R|^2 \NT^2} \,, \\
    &= \frac{1}{|R|} \cdot \frac{m \cdot \mix \cdot \nt_{\emax}}{\eps^2 \NT} \,, \\
    &\leq  \frac{1}{c\log n} \,,
\end{align*}
where the last inequality follows by the choice of $r=|R|$.
\end{proof}

\subsection{Analysis of \textsc{EdgeCountEstimator}}

In this section, we show that the \textsc{EdgeCountEstimator}
procedure (~\Cref{alg:edge_estimate}) has provable 
guarantees. However, we emphasize that, \textsc{EdgeCountEstimator}
together with \ALG works much better than what 
the theoretical bounds suggests.
\begin{theorem}
\label{thm:edge_estimator}
Let $\eps >0$ be some constant and
$r=O(\frac{1}{\eps^2}\cdot \mix \cdot \sqrt{m})$. Then, \textsc{EdgeCountEstimator} outputs $\overline{m}$ such that 
$\overline{m} \in [(1-\eps)m,(1+\eps)m]$ with high probability.
\end{theorem}
\begin{proof}
The proof of the theorem follows from the application of 
~\Cref{thm:collision} and
First observe that the edges in the collection $R$ that are $\mix$ distance apart are independent~\cite{lovasz1993random}. 
Hence, each set $R_i$,
as defined on~\cref{line:R_i)} of~\Cref{alg:edge_estimate},
consists of uniform random edge samples. The theorem now
follows by the size bound given in~\Cref{thm:collision}.
\end{proof}

